On the Limitations of Elo: Real-World Games, are Transitive, not Additive

Real-world competitive games, such as chess, go, or StarCraft II, rely on Elo models to measure the strength of their players. Since these games are not fully transitive, using Elo implicitly assumes they have a strong transitive component that can correctly be identified and extracted. In this study, we investigate the challenge of identifying the strength of the transitive component in games. First, we show that Elo models can fail to extract this transitive component, even in elementary transitive games. Then, based on this observation, we propose an extension of the Elo score: we end up with a disc ranking system that assigns each player two scores, which we refer to as skill and consistency. Finally, we propose an empirical validation on payoff matrices coming from real-world games played by bots and humans.

==> sections/3_proposed_approach_old.tex <==
% !TEX root = ../417.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proposed approach}
\label{sec:proposed_approach}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \quentin{insist on contribs}
We now present our main contribution, which is threefold:
\begin{itemize}[noitemsep,itemjoin = \quad,topsep=0pt,parsep=0pt,partopsep=0pt, leftmargin=*]
    % ,label=(\alph*)
    \item
    We first throughly study the disc game, $\payoffprob{i}{j}
    =
    \sigma(\player{i} \playerv{j} - \playerv{i} \player{j}) \,, \quad i,j \in [n]$  (\Cref{ex:disc_game}).
    We show that depending on the value of $\vect{u}$ and $\vect{v}$,
    % the distribution of players,
    the disc game is either transitive or cyclic (\Cref{prop:disc_game,prop:positive_trans}).
    \item Then, in \Cref{sec:theoretical_analysis} we show that any empirical matrix from real-world zeros-sum games can be decomposed as a sum of empirical disc games, with \emph{at most} one transitive empirical disc game (\Cref{thm:at_most_one_transitive}).
    This motivates our disc rating system which corresponds to the extraction of the empirical matrix's main component (disc game).
    If this main component corresponds to a transitive (resp. cyclic) disc game, then the original game is mainly transitive (resp. cyclic).
    \item Finally in \Cref{sub:optimization_details} we provide the optimization details used to compute the proposed extension of the Elo score (\Cref{alg:otho_decomp}).
\end{itemize}
% \begin{itemize}[noitemsep,itemjoin = \quad,topsep=0pt,parsep=0pt,partopsep=0pt, leftmargin=*]
%     % ,label=(\alph*)
%     \item We first study an example in between the transitive Elo game and the cyclic disc game: the empirical disc game (\Cref{ex:ctr_disc_game}, in \Cref{sub:cstr_disc_game}).
%     We show that depending on the (empirical) distribution of players, the empirical disc game is either transitive or cyclic (\Cref{prop:disc_game,prop:positive_trans}).
%     \item Then, in \Cref{sec:theoretical_analysis} we show that any empirical matrix from real-world zeros-sum games can be decomposed as a sum of empirical disc games, with \emph{at most} one transitive empirical disc game (\Cref{thm:at_most_one_transitive}).
%     This motivates our disc rating system which corresponds to the extraction of the empirical matrix's main component (disc game).
%     If this main component corresponds to a transitive (resp. cyclic) disc game, then the original game is mainly transitive (resp. cyclic).
%     \item Finally in \Cref{sub:optimization_details} we provide the optimization details used to compute the proposed extension of the Elo score (\Cref{alg:otho_decomp}).
% \end{itemize}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Detail Study of the Disc Game}
\label{sub:cstr_disc_game}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The formulation of the cyclic disc game in \Cref{ex:disc_game} is \emph{fully cyclic}. However, in this section, we show that, in general, the empirical version
of the disc game
\begin{equation}
\label{ex:ctr_disc_game}
    \vect{u},\vect{v} \in \sR^n
    \: \text{ and } \:
    \payoffprob{i}{j}
    =
    \sigma(\player{i} \playerv{j} - \playerv{i} \player{j}) \,, \, i,j \in [n]\,,
\end{equation}
\looseness=-1
can either be \emph{fully cyclic} or \emph{fully transitive}  (see \Cref{prop:disc_game}), depending on the of the values of $(\player{i},\playerv{i})$.
\quentin{
    This idea is at the core of our contribution: when studying a real world game, players usually try to win the game; they only pick strategies that seem optimal for them.
Only a specific set of strategies is practically played, thus \emph{one cannot consider a game and its players separately}.
For instance, if the empirical distribution $(\player{i},\playerv{i})$ corresponds to $\player{i} \in \sR$ and $\playerv{i}=1$, then one recovers a transitive Elo game.
One can see that depending on the empirical distribution of $(\player{i}, \playerv{i})$, the empirical disc game can either be transitive ($\playerv{i}=1$) or cyclic (Example~\ref{ex:disc_game}).
One can show that, under mild assumptions, an empirical disc game is either fully transitive or fully cyclic.
}
\quentin{to rephrase0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{propositionrep}[An Empirical Disc Game is Fully Cyclic or Fully Transitive]
    \label{prop:disc_game}
    Let $\vect{u}, \vect{v} \in \sR^n$ and
    $\payoffprob{i}{j}
    =
    \sigma(\player{i} \playerv{j} - \playerv{i} \player{j})\,,\; i,j \in [n]$ be an empirical disc game.
    Let $U:= \hull\{\player{i},\playerv{i}\}$ be the convex hull of the players. If $(0,0)$ is \emph{not} in the border of $U$,\footnote{if it is the case we can, for instance, apply an infinitesimal perturbation on the points $(\player{i},\playerv{i})$.}
    then the empirical disc game is either fully transitive or fully cyclic. Precisely,
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{enumerate}
        \item The empirical disc game is cyclic if and only if $(0,0) \in \Int(U)$.
        \item Otherwise, the empirical disc game is transitive.
    \end{enumerate}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{propositionrep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{appendixproof}
Let us start this proof by showing that there always exists a cycle a size $3$ in a larger cycle.
\begin{lemma}[A cycle of size $n$ implies a cycle of size 3]
If there exists $\player{1},\ldots,\vect{u}_n \in U$ such that $\player{1} \xrightarrow{\!\mathrm{beats}\!} \ldots  \xrightarrow{\!\mathrm{beats}\!} \vect{u}_n \xrightarrow{\!\mathrm{beats}\!} \player{1}$, then there exists $u,v,w \in U$ such that $u \xrightarrow{\!\mathrm{beats}\!} v \xrightarrow{\!\mathrm{beats}\!} w \xrightarrow{\!\mathrm{beats}\!} u$.
\end{lemma}
\begin{proof}
We will use a recursive argument. It is true for $n=3$. Let us assume it is true for a given $n \in \sN$, then given $\player{1} \xrightarrow{\!\mathrm{beats}\!} \ldots  \xrightarrow{\!\mathrm{beats}\!} \vect{u}_{n+1} \xrightarrow{\!\mathrm{beats}\!} u_1$ we have two possible cases
\begin{enumerate}
    \item $\player{1} \xrightarrow{\!\mathrm{beats}\!} \vect{u}_n  \xrightarrow{\!\mathrm{beats}\!} \vect{u}_{n+1} \xrightarrow{\!\mathrm{beats}\!} \player{1}$:
    In that case we have proved the result.
    \item $\player{1} \xleftarrow{\!\mathrm{beats}\!} \vect{u}_n \xrightarrow{\!\mathrm{beats}\!} \vect{u}_{n+1} \xrightarrow{\!\mathrm{beats}\!} \player{1}$.
    In that case is means that  $\player{1} \xrightarrow{\!\mathrm{beats}\!} \ldots  \xrightarrow{\!\mathrm{beats}\!} \vect{u}_{n} \xrightarrow{\!\mathrm{beats}\!} \player{1}$ and thus we can use the recurrence hypothesis that there exists a cycle of size $3$ inside a cycle of size $n$.
\end{enumerate}
\end{proof}

We can now show Proposition~\ref{prop:disc_game}.

The idea of the proof is to use the polar coordinates for all the points $(\player{i},\playerv{i})=(r_i,\theta_i)\in \sR^2$. We can notice that $\payoffprob{i}{j} = \sigma(\player{i} \playerv{j} - \playerv{i} \player{j}) = \sigma(r_i r_j \sin(\theta_i - \theta_j))$. Thus $\payoffprob{i}{j}>1/2$ if and only if $\theta_j + \pi >\theta_i> \theta_j$.
If the game is cyclic it mean that there exists a cycle of size 3. Without any loss of generality let us assume $\theta_1=0$. Then we have that $\pi>\theta_2>0$ and $-\pi<\theta_3<0$. Finally the fact that $\theta_3<\theta_2+\pi$ implies that either $\theta_2>\pi/2$ or $\theta_3 <\pi/2$. Thus this form a triangle that contains $(0,0)$.
Thus we can show that $(0,0)$ is in the interior of the convex set defined by three points of the cycle. If $(0,0)$ is in the interior of $U$ then we can find a cycle.
% Similarly, when we consider
\end{appendixproof}
% In this proposition $\Int(U)$ is the interior\footnote{Roughly the interior of $U$ is the set of points that are not in the border of $U$, more formally, $x \in \Int(U) \Leftrightarrow \exists \epsilon >0 \,,\, \text{s.t.} \,,\, B(x,\epsilon) \subset U$} of $U$.
The main takeaway from this result is that the convex hull of the players $U$ is the crucial element in assessing if an empirical game is transitive or cyclic. The dichotomy happens around the origin.

\begin{propositionrep}[Reparametrization]
\label{prop:positive_trans}
Let $\vect{u},\vect{v} \in \sR^n $ and
    $\payoffprob{i}{j}
    :=
    \sigma(\player{i} \playerv{j} - \playerv{i} \player{j})\,,\; i,j\in [n]$ be a \textbf{transitive} empirical disc game. There exists a reparametrization of the disc game $(\tilde {\vect{u}}_i,\playertildev{i})$ such that, for all $i \in [n]$, $ \playertildev{i} > 0$, and
    \begin{equation}
        \sigma(
            \player{i} \playerv{j} - \playerv{i} \player{j}
            )
        = \payoffprob{i}{j}
        =
        \sigma(
            \tilde{\vect{u}}_i \tilde{\vect{v}}_j - \playertildev{i} \tilde{\vect{u}}_j)
    \enspace .
    % \quad \text{and} \quad
    % \playertildev{i} > 0 \,,\; i \in [n]\,.
    \end{equation}
\end{propositionrep}
\begin{appendixproof}
To prove this result we will use \Cref{prop:disc_game}. Since the empirical disc game is considered transitive and that $(0,0)$ is not in the border of $U$, we know that $(0,0) \notin U = \hull \{(\player{i},\playerv{i})\}$. Thus, by the hyperplane separation theorem~\citep[Example 2.20]{boyd2004convex} there exists a direction $a \in \sR^2\,,\; \|a\|_2=1$ such that, $\langle a,[\player{i},\playerv{i}]\rangle >0\,,\; \forall i \in [n]$. Setting $b := [a_2, -a_1]$, we get that $(a,b)$ is an orthonormal basis of $\sR^2$. Let $(\tilde{\vect{u}}_i,{\vect{v}}_i):= (\langle a,[\player{i},\playerv{i}]\rangle, \langle b, [\player{i},\playerv{i}])$ be the coordinate of $[\player{i},\playerv{i}]$ in this new basis. Finally, we just need to remark that $\player{i} \playerv{j} - \playerv{i} \player{j}$ does not depend on the choice of basis. It is because,  $\player{i} \playerv{j} - \playerv{i} \player{j} = \sigma(\|OM_i\|\|OM_j\| \sin \widehat{M_iOM_j})$ where $M_i \in \sR^2$ corresponds to the point with coordinate $[(\player{i},\playerv{i})]$.
\end{appendixproof}
The proof of this result relies on \Cref{prop:disc_game} and the hyperplane separation theorem~\citep[Example 2.20]{boyd2004convex}.
Because the reparametrization $(\tilde {\vect{u}}_i,\playertildev{i})$ yields the same payoffs, it corresponds to the same disc game.
\Cref{prop:positive_trans} means that, without any loss of generality, one can consider that $\playerv{i} >0\,,\; i \in [n]$ for any transitive empirical disc games.
In the next section, we will see that any empirical payoff $\rmP$ (\Cref{def:empirical_game}) can be transformed into a skew-symmetric matrix $\rmA$ and decomposed as a sum of empirical disc games. We will then use~\Cref{prop:disc_game} on the main empirical disc game to assess the transitivity/cyclicity of the original empirical game $\rmA$.
% \emph{another take} on how to empirically study real world games.  More precisely, in order to take into account the fact that the agents who play the game have limited compute and memory they cannot play the optimal policies.


% \quentin{[Note: show that if $0$ is in cvx hull, then the whole game is cyclic]}



% is composed of several steps until a final state is reached.
% In that game a strategy

% [[continue here and clarify that]
% \begin{definition}[Informal] We say that a game is (articulated transitive and cyclic)
% \begin{enumerate}
%     \item Cyclic: if there exists $u,v,w \in U$ such that $u \xrightarrow{\!\mathrm{beats}\!} v \xrightarrow{\!\mathrm{beats}\!} w \xrightarrow{\!\mathrm{beats}\!} u$,  $\quad u \succeq v$.
%     \item Transitive: if for all $u,v,w \in U$, we have ($u \xrightarrow{\!\mathrm{beats}\!} v$ and $v \xrightarrow{\!\mathrm{beats}\!} w $)  $ \Longrightarrow u \xrightarrow{\!\mathrm{beats}\!} w$.
% \end{enumerate}
% \end{definition}

% \begin{proposition}[A cycle of size $n$ implies a cycle of size 3] (NOTE: probably known maybe cite someone)
% If there exists $u_1,\ldots,u_n \in U$ such that $u_1 \xrightarrow{\!\mathrm{beats}\!} \ldots  \xrightarrow{\!\mathrm{beats}\!} u_n \xrightarrow{\!\mathrm{beats}\!} u_1$, then there exists $u,v,w \in U$ such that $u \xrightarrow{\!\mathrm{beats}\!} v \xrightarrow{\!\mathrm{beats}\!} w \xrightarrow{\!\mathrm{beats}\!} u$.
% \end{proposition}
% \begin{proof}
% We will use a recursive argument. It is true for $n=3$. Let us assume it is true for a given $n \in \sN$, then given $u_1 \xrightarrow{\!\mathrm{beats}\!} \ldots  \xrightarrow{\!\mathrm{beats}\!} u_{n+1} \xrightarrow{\!\mathrm{beats}\!} u_1$ we have two possible cases
% \begin{enumerate}
%     \item $u_1 \xrightarrow{\!\mathrm{beats}\!} u_n  \xrightarrow{\!\mathrm{beats}\!} u_{n+1} \xrightarrow{\!\mathrm{beats}\!} u_1$: In that case we have proved the result.
%     \item $u_1 \xleftarrow{\!\mathrm{beats}\!} u_n \xrightarrow{\!\mathrm{beats}\!} u_{n+1} \xrightarrow{\!\mathrm{beats}\!} u_1$. In that case is means that  $u_1 \xrightarrow{\!\mathrm{beats}\!} \ldots  \xrightarrow{\!\mathrm{beats}\!} u_{n} \xrightarrow{\!\mathrm{beats}\!} u_1$ and thus we can use the recurrence hypothesis that there exists a cycle of size $3$ inside a cycle of size $n$.
% \end{enumerate}
% \end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Theoretical Analysis}
\label{sec:theoretical_analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The empirical version of this game is given a population $(u_i)_{1\leq i \leq n}$ the matrix game
% \begin{equation}
%     \min_{x \in \Delta_n} \max_{y \in \Delta_n} x^\top A y
%     \enspace ,
% \end{equation}
% where $A_{ij} = \varphi(u_i,u_j)$.
%
% In the following, we will try to understand the properties of the matrix game $A$.
First we recall a standard result on the decomposition of skew-symmetric matrices (\Cref{thm:antisym_pca}): any real skew-symmetric matrix can be decomposed as a sum of matrices of the form
$\vect{u} \vect{v}^\top - \vect{v} \vect{u}^\top$,
$\vect{u}, \vect{v} \in \sR^n$.
%, which is usually called the real normal form of an a skew-symmetric matrix~\citep[\S8.16]{greub1975linear}.
Combining this result with \Cref{prop:disc_game}, we finally show that zero-sum game payoff matrices have at most a single transitive disc game component (\Cref{thm:at_most_one_transitive}).

%\looseness-1
%The two main examples of skew-symmetric matrices $\payoffanti{}{}$ arising from empirical probability matrices
%$\payoffprobmat$ are:
%    $\payoffanti{i}{j}
%    =
 %   2 \payoffprob{i}{j} - 1$
  %  and
   % $\payoffanti{i}{j}
    % =
    % \logit \payoffprob{i}{j}$.
%These skew-symmetric matrices are at the core of the proposed score (see \Cref{thm:antisym_pca,thm:at_most_one_transitive}).
%Real skew-symmetric matrices can be decomposed as following.
\begin{theoremrep}\emph{(Normal Decomposition, \citealt{greub1975linear}).}
    \label{thm:antisym_pca}
    Suppose $\mat{A} \in \sR^{n \times n}$ is such that $\payoffanti{}{} = - \payoffanti{}{}^\top$.
    Then, with $k = \floor{n/2}$, there exists
    $\lambda_1 \geq \ldots \geq \lambda_k$
    and
    $(\vect{u}^{(l)}, \vect{v}^{(l)}) \in \sR^n \times \sR^n
    \,,\,1
    \leq
    l
    \leq
    k$,
    such that $(\vect{u}^{(l)}, \vect{v}^{(l)})$ is an orthonormal family and
    % \begin{equation}
        $\mat{A}
        =
        \sum_{l=1}^{k} \lambda_l
             (
            \vect{u}^{(l)} \vect{v}^{(l) \top}
            - \vect{v}^{(l)} \vect{u}^{(l) \top} ) $.
    %     % \label{eq:orth_decomp}
    % \end{equation}

\end{theoremrep}
\begin{appendixproof}
    Proof of \Cref{thm:antisym_pca} can be found in \citet[Sec. 2.5]{cassiniAlgebre3} or \citep[\S8.16]{greub1975linear}.
\end{appendixproof}
% \quentin{comment on the non-unicity?}
%
A proof of \Cref{thm:antisym_pca} can be found in \citet[Sec. 2.5]{cassiniAlgebre3}.
\Cref{thm:antisym_pca} is sometimes referred to as the Schur decomposition of skew-symmetric matrices \citep[Prop. 2]{Balduzzi2018}.
%In the context of empirical games, the theorem has several consequences.
\citet{Balduzzi2019} proposed to compute the normal decomposition of $A$ and visualize it as $2$-dim embeddings but did not provide theorems or insights to interpret it.
\citet{Balduzzi2018} based their $m$-Elo score on this decomposition.
Once the Elo score $\rvu$ is computed, they compute the normal decomposition of the payoff matrix $\rmA - (\rvu \mathbf{1}^\top - \mathbf{1} \rvu^\top)$.
In this work we instead propose to directly compute the normal decomposition of $\rmA$ and provide a principled result (\Cref{thm:at_most_one_transitive}) to interpret its main component in terms of transitivity of the induced disc game. Moreover, we show how to handle missing and infinite (when the probability of winning is $0$ or $1$ the logit is infinite) entries (\Cref{sub:optimization_details}).
%
\rebutal{In the context of symmetric zero-sum games, the first takeaway of Theorem~\ref{thm:antisym_pca} is that
such a game is a sum of disc games.
The second consequence is less obvious but maybe even more important:
among all these discs games \emph{at most one} is transitive.}
%
%
    \begin{theoremrep}[An Empirical Disc Game has at most a Single Transitive Game]
        \label{thm:at_most_one_transitive}
        Let $\mat{P}$ be the payoff matrix of a symmetric zero-sum game, and let $(\vect{u}^{(l)}, \vect{v}^{(l)}) \in \sR^{n} \times \sR^{n} $ be the normal decomposition of the skew-symmetric matrix $\logit(\mat{P})$ (\Cref{thm:antisym_pca}), then there exists \emph{at most} one pair $(\vect{u}^{(l)}, \vect{v}^{(l)}) \in \sR^{n} \times \sR^{n} $ such that the disc game defined by
                $\payoffprob{i}{j} =
                    \sigma(\player{i}^{(l)} \playerv{j}^{(l)}
                    - \playerv{i}^{(l)} \player{j}^{(l)} )$,
        $i, j \in [n]$,
        is transitive.
    \end{theoremrep}
    %
    \begin{appendixproof}
    \rebutal{
    The proof of \Cref{thm:at_most_one_transitive} relies on
    \begin{itemize}
        \item  The  fact that $(\vect{u}^{(l)}, \vect{v}^{(l)})$ are orthogonal.
        \item The reparametrization property (\Cref{prop:positive_trans}).
    \end{itemize}}
    \rebutal{
    The normal decomposition $(\vect{u}^{(l)}, \vect{v}^{(l)})$ is composed of orthogonal vectors ($\vect{v}^{(l)}$ are orthogonal to each others and to $\vect{u}^{(l)}$).}

    \rebutal{
    Suppose that there exist $2$ transitive pairs of components, $(\vect{u}^{(1)}, \vect{v}^{(1)})$ and $(\vect{u}^{(2)}, \vect{v}^{(2)})$. Using  \Cref{prop:positive_trans} we consider the reparametrization such that $\playerv{i}^{(1)} > 0$, for all $i \in [n]$, and $\playerv{i}^{(2)} > 0$, for all $i \in [n]$, hence one has $\vect{v}^{(1) \top } \vect{v}^{(2)} > 0$.
    In addition, since $\vect{v}^{(1)}$ and $\vect{v}^{(2)}$ are orthogonal we have that $\playerv{i}^{(1) \top } \playerv{i}^{(2)} = 0$, which yields a contradiction.
    Hence there exists at most one  transitive pairs of components.}
    % And the fact that is a component $(\vect{u}^{(l)}, \vect{v}^{(l)})$ is transitive then with any loss of generality one can consider that $\playerv{i}^{(l)} > 0$, for all $i \in [n]$.
    \end{appendixproof}
%
\Cref{thm:at_most_one_transitive} provides us with multiple insights.
If one has access to an empirical probability matrix $\mat{P}$, and one can compute the normal decomposition (\Cref{thm:at_most_one_transitive}) of the skew-symmetric matrix $\logit(\mat{P})$,
then the largest value $\lambda_1$ and its associated vectors $(\vect{u}^{(1)}, \vect{v}^{(1)})$ encapsulate information on the largest component.
If the disc game associated with the largest component is transitive, we will say that the considered game based on the empirical probability matrix $\mat{P}$ is transitive.
Note that \Cref{thm:at_most_one_transitive} can be generalized to any invertible functions $f$ which transforms zero-sum game payoff matrices into skew-symmetric matrices, such as for instance $f:\mat{P} \mapsto 2 \mat{P} - 1$.
%
%
\Cref{sub:optimization_details} details main component computation when dealing with real data (i.e., missing and inexact entries).
%  Finally, in \Cref{sec:experiments} we visualize the main empirical disc games of many real-world games. Notably, we show that, according to our visualizations, chess is more transitive than StarCraft II.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computational Details}
\label{sub:optimization_details}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Consider a game $(\varphi, (u_i))$, let $P$ be the payoff matrix, defined as $P_{i, j} = \phi(i, j)$, for all $i, j \in \{1, \dots,  n \}$
Now we provide the details to compute the proposed score.
Consider an empirical probability matrix $(\payoffprob{i}{j})_{\leq i,j \leq n}$.
One can compute the decomposition of $\logit(\vect{P})$ from \Cref{thm:antisym_pca} by solving the following optimization problem, with $\mathcal{L} : \sR \times \sR \rightarrow \sR$, $\mathcal{L}: x, \hat x \mapsto \norm{\logit(x) - \hat x}^2$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
    &\min_{\vect{u}^{(l)}, \vect{v}^{(l)} \in \sR^n}
    f  (\vect{u}, \vect{v})
    \triangleq
     \mathcal{L} (\mat{P}, {\textstyle\sum_{l = 1}^k}\vect{u}^{(l)} {\vect{v}^{(l)}}^\top - \vect{v}^{(l)} {\vect{u}^{(l)}}^\top)
     \nonumber
    \\
     & \quad \quad \quad \quad \quad \quad \triangleq
    \sum_{i, j,l}
     \mathcal{L}(\payoffprob{i}{j}, \player{i}^{(l)} \playerv{j}^{(l)} - \playerv{i}^{(l)} \player{j}^{(l)})
    \enspace ,
    \label{eq:opt_pb_decomposition_gen}
    \\
    & \text{s. t.} \quad
        \langle \vect{u}^{(l)}, \vect{v}^{(l)}\rangle  = 0 \,,\quad
        \langle \vect{u}^{(l)}, \vect{u}^{(m)}\rangle  = \langle \vect{v}^{(l)}, \vect{v}^{(m)}\rangle  = 0\,,\quad 1\leq l < m \leq k\, \enspace .
        \nonumber
\end{align}
% \begin{minipage}[t]{0.52\linewidth}
    \begin{algorithm}[t]
        \caption{Alternate minimization}
        \label{alg:altmin}
        \SetKwInOut{Input}{input}
        \SetKwInOut{Init}{init}
        \SetKwInOut{Parameter}{param}
        \Input{$\mat{A} \in \sR^{n \times  n},
            \mat{us}, \mat{vs} \in \sR^{n \times  k}, l \in \mathbb{N}$}
        \Init{$\vect{u}, \vect{v} \neq 0_{n}$}
        \For{$k = 1, 2 \dots, $}
        {
        $\vect{u} \leftarrow \argmin_{\vect{u}}
        \mathcal{L}(\mat{P}, \mat{A} + \vect{u} \vect{v}^\top - \vect{v} \vect{u}^\top)
        $
        \\
        $
        +
        \sum_{m=1}^{l-1} \frac{\langle \vect{u}, \vect{vs}_{:m} \rangle^2}{\normin{\vect{vs}_{:m} }^2 }
        +
        \sum_{m=1}^{l-1} \frac{\langle \vect{u}, \vect{us}_{:m} \rangle^2}{\normin{\vect{us}_{:m} }^2 }
        $

        $\vect{v} \leftarrow
        \argmin_{\vect{v}}
         \mathcal{L}(\mat{P}, \mat{A} + \vect{u} \vect{v}^\top - \vect{v} \vect{u}^\top)
        + \tfrac{\langle \vect{u}, \vect{v} \rangle^2}{\normin{\vect{u}}^2 }
        $
        \\
        $
        +
        \sum_{m=1}^{l-1} \tfrac{\langle \vect{v}, \vect{vs}_{:m} \rangle^2}{\normin{\vect{vs}_{:m} }^2 }
        +
        \sum_{m=1}^{l-1} \tfrac{\langle \vect{v}, \vect{us}_{:m} \rangle^2}{\normin{\vect{us}_{:m} }^2 }
        $
        % \tcp*[r]{$\bigo(np)$}
        }
    \Return{$\vect{u}, \vect{v}$}
    \end{algorithm}
%
\rebutal{One challenge of this optimization problem is to maintain the orthogonality constraint between the components.} We propose~\Cref{alg:otho_decomp} which sequentially finds the $l^{th}$ main components $(\vect{u}^{(l)}, \vect{v}^{(l)})$ for $l \in [k]$.
The $l^{th}$ pair of components is found with~\Cref{alg:altmin} which maintains the orthogonality constraints by using a penalty term (inspired by the algorithm of~\citet{Gemp2021} which computes PCA for large scale problems).
Note that in practice, empirical probability matrices can have $0$ or $1$ entries, for which $\logit$ is not defined.
That's why in practice (\Cref{sec:experiments}) we use the following loss function
 $\mathcal{L} : x, \hat x \mapsto \mathrm{bce}(x, \sigma(\hat x))$ (where $\mathrm{bce}$ is the binary cross entropy).
Note that the optimization problem formulations based on \Cref{eq:opt_pb_decomposition_gen} can handle missing entries as in \citet{CandesRecht2008,CandesPlan2009}, \rebutal{see the missing entries paragraph in \Cref{app:computational_details} for details}.
%
%
% \begin{minipage}[t]{0.44 \linewidth}
    \begin{algorithm}[tb]
        \caption{Compute disc decomposition}
        \label{alg:otho_decomp}
        \SetKwInOut{Input}{input}
            \SetKwInOut{Init}{init}
            \SetKwInOut{Parameter}{param}
             \Input{$k \in \mathbb{N}$ \textcolor{blue}{($\#$ of pairs of components)}}
             \Init{$\mat{A} = 0_{n \times n}$, \\
             $\mat{us} = 0_{n \times  k}$,
             $\mat{vs} = 0_{n \times  k}$
             }
            \For{$l = 1, 2, \dots, K$ }{
                $\vect{u}^{(l)}, \vect{v}^{(l)} = \mathrm{\Cref{alg:altmin}}(\mat{A}, \mat{us}, \mat{vs}, l)$

                $\mat{A} \leftarrow \mat{A} + \vect{u}^{(l)}  \vect{v}^{(l) \top}  - \vect{v}^{(l)} \vect{u}^{(l) \top} $

                $\mat{us}_{: l}, \mat{vs}_{: l}
                = \vect{u}^{(l)}, \vect{v}^{(l)}$
            }
        \Return{$(\vect{u}^{(l)}, \vect{v}^{(l)})_{1 \leq l \leq k}$}
    \end{algorithm}
    % \end{minipage}
\begin{figure}[tb]
    % \begin{minipage}{0.26 \linewidth}
        {    \centering
    \includegraphics[width=0.95\linewidth]{figures/elo_break_extended_elo.pdf}
    }
% \end{minipage}
% \hfill
% \begin{minipage}{0.7 \linewidth}
    \caption{
        \textbf{\Ours manages to rank players for some transitive games.}
        The logit of the probability of winning,
        $\player{1} \playerv{2} - \playerv{1} \player{2}$, computed
        using the stationary \ours (in \Cref{eq:opt_pb_decomposition_gen}) is displayed for multiples probability matrices of the transitive game (\Cref{ex:trans_non_elo}.
        Red dots indicate that $ \player{1} \playerv{2} - \playerv{1} \player{2} <0$, and green dots $ \player{1} \playerv{2} - \playerv{1} \player{2} > 0$.
        The size of the dots is proportional to $ |\player{1} \playerv{2} - \playerv{1} \player{2}|$.
        Contrary to the Elo score (\Cref{fig:elo_break}), the proposed \ours can correctly rank player $1$ and $2$.
    }
    \label{fig:extended_elo_works}
% \end{minipage}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\textbf{Interpretation of the \ours in the case $k=1$.}
With the proposed \ours, based on two scalars $(\player{i}, \playerv{i})$ per player, the probability of the outcome of new matchups is given by $\sigma(\player{i} \playerv{j} - \playerv{i} \player{j})$.
If it occurs that $j$, $\playerv{j} > 0$, which corresponds to a transitive game (see \Cref{thm:at_most_one_transitive} and \Cref{prop:positive_trans}), then the outcome probability can be written as
$\sigma(\player{i} \playerv{j} - \playerv{i} \player{j})=
\sigma  (\playerv{i} \playerv{j}  ( \player{i} / \playerv{i} -  \player{j} / \playerv{j} ) ) $.
For a player $i$, the ratio
$ \playertilde{i} = \player{i} / \playerv{i}$
 can be interpreted as its \emph{strength}, and $v_i$ as its \emph{consistency} to beat lower rated players (and be beaten by higher rated players): the larger $\playerv{i}$, the larger the probability to win against a lower rated player ($\playertilde{i}  > \playertilde{j} $), but the larger the probability to lose against a higher rated player ($\playertilde{i}  < \playertilde{j} $). This consistency score can be seen as a way to correct the Elo score which implicitly assumes that the strength of each player is linearly comparable in the logit space.
 For instance, one implicit bias of the Elo score is that if $i$ beats $j$ with probability $\mat{P}_{ij}$ and $j$ beats $k$ with probability $\mat{P}_{jk}$ then $i$ beats $k$ with probability
 $\logit(\mat{P}_{ik}) =
 \logit(\mat{P}_{ij})
 +
 \logit(\mat{P}_{jk})$.
%  \geq \max(\mat{P}_{ab}, \mat{P}_{bc})$.
 As illustrated in \Cref{ex:trans_non_elo} if such a property of additivity in the logit space is not occurring in the data, the Elo score may have trouble to even predict the right ranking for the players (\Cref{fig:elo_break}). Conversely, when including a notion of \emph{consistency} in our score we manage to correctly predict the ranking between the players in~\Cref{ex:trans_non_elo} (see~\Cref{fig:extended_elo_works}.)

\textbf{Online update.}
The main focus of this work is to study the intrinsic characteristics of the game at a given time $t$.
This is opposed to the line of work that considers the games sequential aspect, quantifying the Elo score uncertainty with a Bayesian model (TrueSkill, \citealt{herbrich2006trueskill}), or relying on the more recent games \citep{Sismanis2010}.
However, an update rule can still be derived and interpreted for the proposed \ours.
%
The stationary version of the proposed disc score is written in \Cref{eq:opt_pb_decomposition_gen}, the online version \citep{Jabin2015} of the \ours writes, with a step size
$\eta >0$,  $\mat{S}_{i j}^t$
the result of the confrontation between players $i$ and $j$,
and
$\payoffprobhat{i}{j}^t
=
\sigma(\playerv{i}^{t} \playerv{j}^{t}(\playertilde{i}^t - \playertilde{j}^t ) )$:
%
\begin{align}
    \playertilde{i}^{t+1}
    &=
    \playertilde{i}^{t}
    + \eta (\mat{S}_{i j}^t - \payoffprobhat{i}{j}^t ) \playerv{i}^{t} \playerv{j}^{t}
    \enspace ,
    \\
    \playerv{i}^{t+1}
    &=
    \playerv{i}^{t}
    + \eta (\mat{S}_{i j}^t - \payoffprobhat{i}{j}^t) \playerv{j}^{t}
    (\playertilde{i}^{t} - \playertilde{j}^{t})
    \enspace .
\end{align}
As for the usual Elo score, the increase of the "strength"
$\playertilde{i}$
after a confrontation is proportional to
$\mat{S}_{i j}^t - \payoffprobhat{i}{j}^t$.
The "consistency" $\playerv{i}$ increases when beating lower-rated players and decreases when losing against lower-rated players. Informally, this quantity encompasses how much one should trust the current Elo score and scales up or down the ``strength'' update.
%

